A Survey on EOSIO Systems Security: Vulnerability, Attack, and Mitigation

EOSIO, as one of the most representative blockchain 3.0 platforms, involves lots of new features, e.g., delegated proof of stake consensus algorithm and updatable smart contracts, enabling a much higher transaction per second and the prosperous decentralized applications (DApps) ecosystem. According to the statistics, it has reached nearly 18 billion USD, taking the third place of the whole cryptocurrency market, following Bitcoin and Ethereum. Loopholes, however, are hiding in the shadows. EOSBet, a famous gambling DApp, was attacked twice within a month and lost more than 1 million USD. No existing work has surveyed the EOSIO from a security researcher perspective. To fill this gap, in this paper, we collected all occurred attack events against EOSIO, and systematically studied their root causes, i.e., vulnerabilities lurked in all relying components for EOSIO, as well as the corresponding attacks and mitigations. We also summarized some best practices for DApp developers, EOSIO official team, and security researchers for future directions.

==> Section-Taxonomy.tex <==
\section{Taxonomy}
\label{sec:taxonomy}

\he{consider to remove this section}

\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tbp]
\centering
\caption{Selected Attack events for each type of vulnerabilities.}
\begin{tabular}{ccc}
\toprule
\textbf{Vulnerability Type}                                                                      & \textbf{Victims}                                                    & \textbf{EOS Loss}   \\ \midrule
asset Overflow                                                                                   & \begin{tabular}[c]{@{}c@{}}zyixjmpxrrpr\\ eosfoiowolfs\end{tabular} & 60,686.40           \\ \midrule
\multirow{5}{*}{Fake EOS}                                                                        & xlotoioeosio                                                        & 34.00               \\ \cline{2-3} 
                                                                                                 & eosbetdice11                                                        & 44,427.40           \\ \cline{2-3} 
                                                                                                 & eosluckydice                                                        & 4,508.00            \\ \cline{2-3} 
                                                                                                 & eoscastdmgb1                                                        & 63,014.10           \\ \cline{2-3} 
                                                                                                 & vegasgame111                                                        & 528.00              \\ \midrule
\multirow{5}{*}{Fake Receipt}                                                                    & nkpaymentcap                                                        & 53,641.60           \\ \cline{2-3} 
                                                                                                 & gambaccarats                                                        & 1,922.60            \\ \cline{2-3} 
                                                                                                 & epsdcclassic                                                        & 17,386.80           \\ \cline{2-3} 
                                                                                                 & pickowngames                                                        & 73.50               \\ \cline{2-3} 
                                                                                                 & eosbetdice11                                                        & 145,321.00          \\ \midrule
\multirow{5}{*}{Flawed Random Numer}                                                             & eosplaybrand                                                        & 29,200.00           \\ \cline{2-3} 
                                                                                                 & rockscissors                                                        & 6,500.00            \\ \cline{2-3} 
                                                                                                 & thebetxowner                                                        & 7,125.60            \\ \cline{2-3} 
                                                                                                 & skreosladder                                                        & 1,211.00            \\ \cline{2-3} 
                                                                                                 & hotbetsadmin                                                        & 1,262.70            \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Permission Verification\\ Vulnerability\end{tabular}} & thedeosgames                                                        & 2,090.00            \\ \cline{2-3} 
                                                                                                 & yumgamescard                                                        & 93.60               \\ \midrule
\multirow{4}{*}{hard\_fail Attack}                                                               & flagshipladd                                                        & 1,997.00            \\ \cline{2-3} 
                                                                                                 & walletclover                                                        & 4,418.00            \\ \cline{2-3} 
                                                                                                 & mercatoxeos1                                                        & 4,815.00            \\ \cline{2-3} 
                                                                                                 & eosvegasgame                                                        & 2,202.50            \\ \midrule
Inline Reflex                                                                                    & fastwindice3                                                        & 1,929.20            \\ \midrule
\multirow{4}{*}{memo Attack}                                                                     & skreosladder                                                        & 6,000.00            \\ \cline{2-3} 
                                                                                                 & eosbluebcrat                                                        & 5,624.00            \\ \cline{2-3} 
                                                                                                 & epsroulettes                                                        & 4,860.00            \\ \cline{2-3} 
                                                                                                 & roulette.e                                                          & 2,399.20            \\ \midrule
\multirow{2}{*}{Replay}                                                                          & eoslotsystem                                                        & 65.70               \\ \cline{2-3} 
                                                                                                 & happyeosslot                                                        & 5,000.00            \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Rollback /\\ Blacklisted Account\end{tabular}}        & vsvsvsbetbet                                                        & 1,028.10            \\ \cline{2-3} 
                                                                                                 & bocai.game                                                          & 709.70              \\ \cline{2-3} 
                                                                                                 & eosbiggame44                                                        & 14,903.20           \\ \cline{2-3} 
                                                                                                 & nutsgambling                                                        & 1,141.70            \\ \cline{2-3} 
                                                                                                 & \begin{tabular}[c]{@{}c@{}}luckygoadmin\\ luckygodice1\end{tabular} & 1,029.00            \\ \midrule
\multirow{3}{*}{Deficient Resource System}                                                       & eidosonecoin                                                        & -                   \\ \cline{2-3} 
                                                                                                 & eosio                                                               & -                   \\ \cline{2-3} 
                                                                                                 & wallet.bg                                                           & -                   \\ \midrule
\multirow{5}{*}{Transaction Congestion}                                                          & skreosladder                                                        & 24,500.00           \\ \cline{2-3} 
                                                                                                 & dicer.e                                                             & 4,194.50            \\ \cline{2-3} 
                                                                                                 & farmeosbank1                                                        & 1,844.70            \\ \cline{2-3} 
                                                                                                 & farmeosbank1                                                        & 4,886.40            \\ \cline{2-3} 
                                                                                                 & eosluckydice                                                        & 1,389.50            \\ \midrule
\textbf{Total}                                                                                       & \textbf{-}                                                          & \textbf{533,963.70} \\ \bottomrule
\end{tabular}
\label{table:selected-attack}
\end{table}
\fi

To cover as many types of vulnerabilities related to EOSIO smart contract as possible, we did a comprehensive investigation from different sources, like  blogs from security companies~\cite{peckshield-blog,slowmist-zone}, forums~\cite{bitcoingambling,eosreddit} and official announcements related to attack events.
After collecting all these information, we manually audit the source code or reverse engineering the Wasm bytecode (if the source code is not available) of the corresponding smart contracts.
Consequently, we conducted 13 types of vulnerabilities related to EOSIO smart contract, we selected some representative attack events (according to the amount of financial loss) and demonstrate them in Table~\ref{table:selected-attack}.
Some other attacks did result in huge financial losses, e.g., private key compromising~\cite{}, malicious price manipulation of third-party tokens~\cite{}. However, they are beyond the scope of this paper, we only focus on the vulnerabilities related to application, data and consensus layers (see Fig.~\ref{fig:structure-eosio}).


To this end, we categorized these vulnerabilities according to in which layer they appear. For example, the immediate cause of fake EOS vulnerability is the incomplete verification of arguments in \texttt{apply}. Thus, the fake EOS vulnerability belongs to the application layer.
We further delved for the root causes for all these vulnerabilities.
All these informations are shown in Fig.~\ref{fig:vulnerabilities-layer}.


\begin{figure*}[tbp]
\centerline{\includegraphics[width=\textwidth]{images/vulnerabilities-layer-2.pdf}}
\caption{The vulnerabilities in EOSIO, and their corresponding locations and causes.}
\label{fig:vulnerabilities-layer}
\end{figure*}












































